Variance on the Leaves of a Tree Markov Random Field: Detecting Character Dependencies in Phylogenies

Stochastic models of evolution (Markov random fields on trivalent trees) generally assume that different characters (different runs of the stochastic process) are independent and identically distributed. In this paper we take the first steps towards addressing dependent characters. Specifically we show that, under certain technical assumptions regarding the evolution of individual characters, we can detect any significant, history independent, correlation between any pair of multistate characters. For the special case of the Cavender-Farris-Neyman (CFN) model on two states with symmetric transition matrices, our analysis needs milder assumptions. To perform the analysis, we need to prove a new concentration result for multistate random variables of a Markov random field on arbitrary trivalent trees: we show that the random variable counting the number of leaves in any particular subset of states has variance that is subquadratic in the number of leaves.

==> lemmaproofs.tex <==
\section{Proofs of Lemma \ref{lem:independent} and \ref{lem:dependent}}\label{sec:lems}
Let $\mu_0$ be the state at the root. Let $r_0 = \mu_0 - \mu$ be the error vector at the root. Recall, $\mu$ is the uniform distribution over the $s^2$ states. 
For a leaf $\ell$, recall that $\mu_\ell$ is the distribution at the leaf, and $r_\ell = \mu_\ell - \mu$. If the characters are independent, then we have $P_e = M_e \otimes N_e$ at every edge. This implies two things: $||P_e|| \leq \lambda < 1$ for some $\lambda$, and $P_e$ is doubly-stochastic since both $M_e$ and $N_e$ are doubly stochastic. Therefore, $\mu$ is a stationary distribution and thus,
\begin{equation}\label{eq:r:independent}
	r_\ell = r_0^\top P_{e_1}P_{e_2}\cdots P_{e_{d(\ell)}}
\end{equation}
where $(e_1,e_2,\ldots,e_{d(\ell)})$ is the path from the root to the leaf $\ell$. By Lemma \ref{lem:fact}, we get $||r_\ell||_1 \leq \lambda^{d(\ell)}||r_0||_1 \leq 2\lambda^{d(\ell)}$ since $||r_0||_1 \leq ||\mu||_1 + ||\mu_0||_1 = 2$. In turn, this implies $|\langle r_\ell,e_i\rangle| \leq 2\lambda^{d(\ell)}$. 

Note for any $i$, we have
$\Exp[Z_i] = \sum_{\ell} \langle \mu_\ell,e_i\rangle = n/s^2 + \sum_\ell\langle r_\ell,e_i\rangle$.
This, along with the bounds from the previous para, gives for any $i$ and $j$, we have $$|\Exp[Z_i] - \Exp[Z_j]| \leq 4\sum_{\ell}^{} \lambda^{d(\ell)} \leq O(n^{1-\log_2(1/\lambda)})$$
where the inequality follows from Claim \ref{claim:bounddelta}. This proves Lemma \ref{lem:independent}.

\subsection{Approach towards Lemma \ref{lem:dependent}.}
For every model of evolution, in Section \ref{sec:models}, we exhibit another vector $r^* \in \R^{s^2}$ whose coordinates sum up to zero with each entry in $[-1,+1]$, such that 
\begin{equation}\label{eq:goal}\tag{{Deviation}}
\textrm{For all $\ell$, we have} \quad \langle r_\ell,r^*\rangle \geq \eps.
\end{equation}
where $\eps$ is a parameter depending on $\delta$ and $s$.   
Let $\bar{\mu} := \frac{1}{n}\sum_{\ell}\mu_\ell$.
Observe that $\langle\bar{\mu},r^*\rangle \geq \eps$ as well. Since $r^*$ is a convex combination of vectors of the form $\{e_i-e_j\}$ where $e_i$ is the indicator vector for pair $i$, we get there exists $(i,j)$ such that $\langle \bar{\mu},(e_i - e_j)\rangle \geq \eps$. But $\langle\bar{\mu},e_i\rangle$ is precisely $\Exp[Z_i]/n$ since $\langle \mu_\ell,e_i\rangle$ indicates the probability leaf $\ell$ is in state $i$. Therefore \eqref{eq:goal} implies that there exists a pair $i$ and $j$ such that  $\Exp[Z_i] - \Exp[Z_j] \geq \eps n.$
This proves Lemma \ref{lem:dependent}.

